Self-Adapting Large Visual-Language Models to Edge Devices across Visual Modalities

Recent advancements in Vision-Language (VL) models have sparked interest in their deployment on edge devices, yet challenges in handling diverse visual modalities, manual annotation, and computational constraints remain. We introduce EdgeVL, a novel framework that bridges this gap by seamlessly integrating dual-modality knowledge distillation and quantization-aware contrastive learning. This approach enables the adaptation of large VL models, like CLIP, for efficient use with both RGB and non-RGB images on resource-limited devices without the need for manual annotations. EdgeVL not only transfers visual language alignment capabilities to compact models but also maintains feature quality post-quantization, significantly enhancing open-vocabulary classification performance across various visual modalities. Our work represents the first systematic effort to adapt large VL models for edge deployment, showcasing up to 15.4% accuracy improvements on multiple datasets and up to 93-fold reduction in model size.

==> sections/introduction.tex <==
\section{Introduction}
Scene classification has been one of the fundamental tasks in computer vision. It aims to predict the scene category of an image, which is a crucial step in indoor scene understanding. Convolutional Networks (CNN) have achieved remarkable success in scene classification \cite{li2018dfltsupgtltsupgtnet}\cite{xiong2021ask}\cite{seichter2022efficient}\cite{caglayan2022when}. However, most of the existing methods focus on the closed vocabulary setting, where the scene categories are fixed.  Recently, large language-vision models such as CLIP \cite{radford2021clip} and ALIGN \cite{jia2021scaling} have learned a shared embedding space by contrastive training with billions of image and text pairs. By measuring the similarities between the image embedding and all candidate text embeddings, one can achieve open vocabulary classification in various computer vision tasks, including image classification \cite{he2022openvocabulary}, semantic segmentation \cite{ghiasi2022scaling} and object detection \cite{minderer2022simple}.

While these large language-vision models have demonstrated remarkable predictive power when integrated into open vocabulary prediction settings, their focus primarily on prevalent RGB images overlooks other critical yet less common modalities such as depth and thermal imaging. For example, depth sensors are often chosen over RGB cameras in indoor environments with poor visibility or for privacy concerns, and thermal cameras are preferred in dark environments. Consequently, there is a need for a versatile open vocabulary scene classification model that can effectively handle different modalities.

On the other hand, large language-vision models are designed to have a large model size and require significant amounts of data in order to enhance their predictive power. But such substantial computational demands make them impractical for use on edge devices, where computational resources are more limited. Model quantization is a common approach to reduce the model size and improve the efficiency of deep neural networks. Quantization methods including LSQ \cite{esser2020lsq}, EWGS \cite{lee2021ewgs} and SmoothQuant \cite{xiao2023smoothquant} have been proposed to quantize the weights and activations of neural networks while maintaining accuracy. However, simply applying these quantization methods to the open vocabulary scene classification model will result in a significant performance drop (See experimental results X.X). It is unknown what the optimum quantization strategy is for open vocabulary scene classification models.

In this work, we address the above issues by proposing \sysname, a knowledge transfer framework for efficient open vocabulary scene classification on edge devices. The proposed \sysname\ consists of two components: (1) a multi-task training strategy that jointly trains the open vocabulary scene classification model with different modalities, and (2) a quantization-aware metric alignment strategy that aligns the metric space of the scene embeddings in the quantized space. The first component aims to transfer the knowledge from large vision models trained on RGB data to other modalities, while the second component ensures the efficiency of the model for deployment on edge devices. Specifically, our contributions are as follows:
\begin{itemize}
  \item We address the open vocabulary scene classification problem on various modalities beyond RGB images, a topic that has not been previously explored.
  \item We investigate the most effective quantization strategy for transferring cross-modal knowledge from large vision models, a novel approach that has not yet been studied.
  \item We will make our training and evaluation code available at \url{http://.../github.com} for open access and reproducibility.
\end{itemize}

% This oversight is inevitably inherited by existing open vocabulary models, which rely on the capabilities of these large vision models. Additionally, the substantial computational demands of large vision models make them impractical for use on edge devices, where computational resources are more limited.

% The open vocabulary setting allows the model to predict a scene category that is not included in the training set. This setting is more practical in real-world applications, as it is impossible to enumerate all possible scene categories. 

